Mean-field analysis for heavy ball methods: Dropout-stability, connectivity, and global convergence

The stochastic heavy ball method (SHB), also known as stochastic gradient descent (SGD) with Polyak's momentum, is widely used in training neural networks. However, despite the remarkable success of such algorithm in practice, its theoretical characterization remains limited. In this paper, we focus on neural networks with two and three layers and provide a rigorous understanding of the properties of the solutions found by SHB: \emph{(i)} stability after dropping out part of the neurons, \emph{(ii)} connectivity along a low-loss path, and \emph{(iii)} convergence to the global optimum. To achieve this goal, we take a mean-field view and relate the SHB dynamics to a certain partial differential equation in the limit of large network widths. This mean-field perspective has inspired a recent line of work focusing on SGD while, in contrast, our paper considers an algorithm with momentum. More specifically, after proving existence and uniqueness of the limit differential equations, we show convergence to the global optimum and give a quantitative bound between the mean-field limit and the SHB dynamics of a finite-width network. Armed with this last bound, we are able to establish the dropout-stability and connectivity of SHB solutions.

==> 2_layers/converge_MF_noisy.tex <==
In this section, we prove the mean-field limit for two-layer neural networks under noisy dynamics. Before going to the proof, we recall the definition of the mean-field ODE and the stochastic heavy ball dynamics. We also similarly define the particle dynamics and the heavy ball dynamics as in noiseless case.

The integral form of the mean-field ODE is defined as follows:
\begin{align}
\label{equ:noisy,MFODE}
    \vtheta(t) = \vtheta(0) - \gamma \int_{0}^{t} (\vtheta(s) - \vtheta(0)) \, ds - \int_{0}^{t} \int_{0}^{s} \nabla_{\vtheta} \Psi_{\lambda}(\vtheta(u); \rho^{\vtheta}(u)) \,du \,ds + \sqrt{2 \gamma \beta^{-1}} \int_{0}^{t} \mB(s) \, ds
\end{align}

The particle dynamics are defined as follows:
\begin{align}
\label{equ:noisy,PD}
    \vthetapd(t,j)  =& \vthetapd(0,j) - \gamma \int_{0}^{t} (\vthetapd(s,j) - \vthetapd(0,j)) \, ds \\
    & - \int_{0}^{t} \int_{0}^{s} \nabla_{\vtheta} \Psi_{\lambda}(\vthetapd(u,j); \rhopd^{\vtheta}(u)) \,du \,ds + \sqrt{2 \gamma \beta^{-1}} \int_{0}^{t} \mB_j(s) \, ds, \forall j \in [n]
\end{align}

where $\rhopd^{\vtheta}(u) = \frac{1}{n} \sum_{i=1}^{n} \delta_{\vthetapd(u)}$ denotes the empirical measure of $\vthetapd_i(u)$, and $\mB_i(t)$ are $n$ i.i.d standard  $(D+1)$-dimensional Brownian motion.

The heavy ball dynamics is defined as follows:
\begin{align}
\label{equ:noisy,HB}
    \vthetahb(k+1,j) = & \vthetahb(k,j) + (1 - \gamma \varepsilon) \big( \vthetahb(k,j) - \vthetahb(k-1,j) \big)\\
    &- \varepsilon^2 \nabla_{\vtheta} \Psi_{\lambda}(\vthetahb(k,j); \rhohb^{\vtheta}(k)) + \sqrt{2 \gamma \beta^{-1}} \mB_j(k \varepsilon), \forall j \in [n]
\end{align}


and the stochastic heavy ball dynamics is defined as follows:
\begin{align}
\label{equ:noisy,SHB}
     \vthetashb(k+1,j) =& \vthetashb_i(k,j) + (1 - \gamma \varepsilon) \big( \vthetashb(k,j)- \vthetashb(k-1,j) \big)\\
     &  - \varepsilon^2 \nabla_{\vtheta} \widehat{\Psi}_{\lambda}(\vz(k),\vthetashb(k,j); \rhoshb^{\vtheta}(k,j)) + \sqrt{2 \gamma \beta^{-1}} \mB_j(k \varepsilon), \forall j \in [n]
\end{align}

where $\rhohb^{\vtheta}(k) $ and $\rhoshb^{\vtheta}(k)$ denotes the empirical measure of the heavy ball dynamics and the stochastic heavy ball dynamics. 

Same as the noisy dynamics, the initialization of (\ref{equ:noisy,PD}), (\ref{equ:noisy,HB}) and (\ref{equ:noisy,SHB})  are the same, which means:
\begin{align*}
    \vthetapd(0,j) = \vthetahb(0,j) = \vthetashb(0,j), \forall j \in [n]
\end{align*}

We comment that in the noisy case, the Brownian motion in (\ref{equ:noisy,PD}), (\ref{equ:noisy,HB}) and (\ref{equ:noisy,SHB}) are also the same , which means the three dynamics are the coupled by the same initialization and the same Brownian noise.

Since the proof for noisy dynamics are similar to the proof for noiseless dynamics, we restate everything again, and just indicate the difference.


% \subsubsection{Bound the mean-field ODE and the particle dynamics }
% \input{2_layers/noisy_MFODE-PD}

% \subsubsection{Bound the particle dynamics and the heavy ball dynamics }
% \input{2_layers/noisy_PD-HB}

% \subsubsection{Bound the heavy ball dynamics and the stochastic heavy ball dynamics}

==> 2_layers/noisy_MFODE-PD.tex <==
In this section, we first similarly define $n$ i.i.d copy of the mean-field dynamics (\ref{equ:noisy,MFODE}) as we do in the noiseless case. 

\begin{align*}
    \vtheta(t,j) = \vtheta(0,j) - \gamma \int_{0}^{t} (\vtheta(s,j) - \vtheta(0,j)) \, ds - \int_{0}^{t} \int_{0}^{s} \nabla_{\vtheta} \Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j)) \,du \,ds + \sqrt{2 \gamma \beta^{-1}} \int_{0}^{t} \mB_j(s) \, ds, \forall j \in [n]
\end{align*}
where $\rho_j^{\vtheta}(u))$ is the law of $\vtheta(u,j)$, and we let the $n$ i.i.d Brownian motion $\mB_j(t)$ to be the same as in the  (\ref{equ:noisy,PD}), which means the two dynamics are coupled by the same initialization and the same Brownian noise.

We have the following results for the noisy dynamics:
\begin{proposition}
\label{prop:noisy,MFODE-PD}
Under assumption \ref{Assum:2L}, we have that:
\begin{align*}
    \dist_T(\vtheta,\vthetapd) \leq  K(\gamma,\lambda,\beta,T) \left[ (\sqrt{1+\log n + \delta^2}) \frac{\log \sqrt{n}T + \delta^2}{ \sqrt{n}} +   \left( D+1+\log n+ \delta^2 \right) \frac{1}{\sqrt{n}} \right] 
\end{align*}
with probability at least $1-6\exp(-\delta^2) $
where $\dist_T(\vtheta, \vthetapd)$ is defined same as the noiseless case in (\ref{equ:dist,2L,MFODE-PD})
\end{proposition}

We first trying to recover the boundedness property of the mean-field ODE and the particle dynamics as in part 2 of Lemma \ref{lemma:priori,2L}. We have the following lemma:
\begin{lemma}
\label{lemma:noisy,bd,MFODE}

Under assumption \ref{Assum:2L} and fix $T>0$, we have that:
\begin{align*}
    \sup_{t \in [0,T]} \max_{j \in [n]} |w_2(t,j)| \leq (K T^2 + 2 T \sqrt{\lambda \beta^{-1} T}) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} T \right)  (\sqrt{1+\log n + \delta^2}) \\
    \sup_{t \in [0,T]} \max_{j \in [n]} \|\vw_1(t,j)\|_2 \leq (K T + 2 T^3 \sqrt{\lambda \beta^{-1} T} ) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} T \right) (\sqrt{D+\log n + \delta^2})
\end{align*}
which implies that:
\begin{align*}
    \sup_{t \in [0,T]} \max_{j \in [n]} \| \vtheta(t,j)\|_2 \leq \leq (K T^2 + 2 T^3 \sqrt{\lambda \beta^{-1} T} ) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} T \right) (\sqrt{D+1+\log n + \delta^2})
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:noisy,bd,MFODE}]
To simplify the notation we define:
\begin{align*}
    m_2(t) = \sup_{s \in [0,t]} \max_{j \in [n]} |w_2(s,j)|,\\
    m_1(t) = \sup_{s \in [0,t]} \max_{j \in [n]} \|w_1(s,j)\|_2 
\end{align*}

By Lemma \ref{lemma:priori,2L,noisy}, we have that:
\begin{align*}
    \| \nabla_{w_2} \Psi_{\lambda} (\vtheta(t,j);\rho^{\vtheta}(t,j)) \|_2 \leq K+\lambda |w_2(t,j)|
\end{align*}
and by the definition of the mean-field dynamics, we have :
\begin{align*}
    |w_2(t,j)| \leq& |w_2(0,j)| + \gamma \int_0^{t} |w_2(s,j)|+|w_2(0,j)| \, ds \\
    & + \int_0^t \int_0^s (K+\lambda |w_2(t,j)|) \, du \,ds  + \left| \int_0^t \sqrt{2 \gamma \beta^{-1}} B(s) \,ds \right|
\end{align*}
which implies that:
\begin{align*}
    m_2(t) \leq &  \max_{j \in [n]}|w_2(0,j)| + \gamma \int_0^{t} m_2(s)+\max_{j \in [n]}|w_2(0,j)| \, ds \\
    & + \int_0^t \int_0^s (K+\lambda m_2(t)) \, du \,ds  + \sup_{t \in [0,T]} \max_{j \in [n]}\left| \int_0^t \sqrt{2 \gamma \beta^{-1}} B_j(s) \,ds \right|
\end{align*}
And now we need to upper bound 
\begin{align}
    \max_{j \in [n]}|w_2(0,j)|, \label{equ:noisy,bd,w_2(0)} \\
    \sup_{t \in [0,T]} \max_{j \in [n]}\left| \int_0^t \sqrt{2 \gamma \beta^{-1}} B_j(s) \,ds \right| \label{equ:noisy,bd,brownian}
\end{align}

For (\ref{equ:noisy,bd,w_2(0)}), by the assumption we have $|w_2(0,j)| \leq K$.

For (\ref{equ:noisy,bd,brownian}), by Lemma \ref{lemma:bd,standard brownian}, we have that:
\begin{align*}
    \sup_{t \in [0,T]} \max_{j \in [n]}\left| \int_0^t \sqrt{2 \gamma \beta^{-1}} B(s) \,ds \right| \leq 2 T \sqrt{\lambda \beta^{-1} T} (\sqrt{1+\log n + \delta^2})
\end{align*}
with probability at least $1-\exp{-\delta^2}$

And the above implies that:
\begin{align*}
     m_2(t) \leq &  (K+KT + K T^2) + \gamma \int_0^{t} m_2(s)\, ds \\
    & + \lambda \int_0^t \int_0^s m_2(u) \, du \,ds  +  2  T\sqrt{\lambda \beta^{-1} T} (\sqrt{1+\log n + \delta^2})
\end{align*}
by Lemma \ref{lemma:Pachatte} implies that:
\begin{align*}
    m_2(t) \leq (K T^2 + 2 T \sqrt{\lambda \beta^{-1} T}) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} t \right)  (\sqrt{1+\log n + \delta^2})
\end{align*}
with probability at least $1-\exp(-\delta^2)$

Next we aim to bound $\|\vw_1(t,j)\|_2$. By Lemma \ref{lemma:priori,2L,noisy}, we have that:
\begin{align*}
    \| \nabla_{\vw_1} \Psi_{\lambda} (\vtheta(t,j);\rho^{\vtheta}(t,j)) \|_2 \leq K|w_2(t,j)|+\lambda \|\vw_1(t,j)\|_2
\end{align*}
which implies that:
\begin{align*}
    m_1(t) \leq &  \max_{j \in [n]}|\vw_1(0,j)| + \gamma \int_0^{t} m_2(s)+ \max_{j \in [n]}|\vw_1(0,j)| \, ds \\
    & + \int_0^t \int_0^s (K m_2(u) +\lambda m_1(u)) \, du \,ds  + \sup_{t \in [0,T]} \max_{j \in [n]}\left| \int_0^t \sqrt{2 \gamma \beta^{-1}} \mB_{j}(s) \,ds \right|
\end{align*}

Thus we need to upper bound: 
\begin{align}
    \max_{j \in [n]}|\vw_1(0,j)|, \label{equ:noisy,bd,w_1(0)}\\
    \sup_{t \in [0,T]} \max_{j \in [n]}\left| \int_0^t \sqrt{2 \gamma \beta^{-1}} \mB_{j}(s) \,ds \right| \label{equ:noisy,bd,brownian,2}
\end{align}

For the (\ref{equ:noisy,bd,w_1(0)}) term, by assumption we have that $\vw_1(0,j)$ are $K$-sub-Gaussian. Thus using the same techniques as in \cite[Lemma 13]{mei2019mean}, we have that:
\begin{align*}
    \max_{j \in [n]} \|\vw_1(0,j)\|_2 \leq 2 K (\sqrt{D+\log N + \delta^2})
\end{align*}
with probability at least $1- \exp(- \delta^2)$

For the (\ref{equ:noisy,bd,brownian,2}) term, from Lemma \ref{lemma:bd,standard brownian}, we have that:
\begin{align*}
     \sup_{t \in [0,T]} \max_{j \in [n]}\left| \int_0^t \sqrt{2 \gamma \beta^{-1}} \mB_{j}(s) \,ds \right| \leq 2 T \sqrt{\lambda \beta^{-1} T} (\sqrt{D+\log n + \delta^2})
\end{align*}
with probability at least $1- \exp(- \delta^2)$

Thus we have:
\begin{align*}
    m_1(t) \leq &  (K T + 2 T^3 \sqrt{\lambda \beta^{-1} T} ) (\sqrt{D+\log n + \delta^2})+ \gamma \int_0^{t} m_1(s) \, ds \\
    & + \lambda\int_0^t \int_0^s  m_1(u)) \, du \,ds  
\end{align*}
with probability at least $1- \exp(- \delta^2)$

Thus we have by Lemma \ref{lemma:Pachatte}:
\begin{align*}
    m_1(t) \leq (K T + 2 T^3 \sqrt{\lambda \beta^{-1} T} ) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} t \right) (\sqrt{D+\log n + \delta^2})
\end{align*}
with probability at least $1- \exp(- \delta^2)$
\end{proof}

We first trying to recover the Lipschitz results as in Lemma \ref{lemma:Lip,MFODE,2L}, we have the following lemma:
\begin{lemma}
\label{lemma:Lip,noisy,2L}
    Under assumption \ref{Assum:2L}, we have the following results for the mean-field dynamics: Fixed $T > 0$, for any $\tau \leq T$
    \begin{align*}
        &\max_{k \in \left[\frac{T}{\tau}\right]} \max_{j \in [n]}  \sup_{h \in[0,\tau]} \| \vtheta(k \tau+h,j) - \vtheta(k \tau,j) \|_2 \leq K(\gamma,\lambda,\beta,T) (\sqrt{D+1+\log n + \delta^2}) \tau  \\
        & \max_{k \in \left[\frac{T}{\tau}\right]} \max_{j \in [n]}  \sup_{h \in[0,\tau]}  \wass_2(\rho^{\vtheta}(k \tau+h,j), \rho^{\vtheta}(k \tau,j)) \leq K(\gamma,\lambda,\beta,T) (\sqrt{D+1+\log n + \delta^2}) \tau
    \end{align*}
    with probability at least $1 - \exp{-\delta^2}$
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lemma:Lip,noisy,2L}]

By the definition of the mean-field dynamics, we have:
\begin{align}
    \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \| \vtheta(t+\tau,j) - \vtheta(t,j) \|_2 \leq \gamma \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \int_{k \tau}^{ k\tau+h} \|\vtheta(s,j) - \vtheta(0,j)\|_2 \, ds \notag\\
    + \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]}\int_{k \tau }^{k \tau + h} \int_{0}^{s} \|\nabla_{\vtheta} \Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j)) \|_2 \, du \, ds \notag\\
    + \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2 \label{equ:Lip,noisy,full}
\end{align}

Clearly we have:
\begin{align*}
    \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \int_{k \tau}^{ k\tau+h} \|\vtheta(s,j) - \vtheta(0,j)\|_2 \, ds \leq \tau \cdot \sup_{t \in [0,T]} \max_{j \in [n]}  \|\vtheta(s,j) - \vtheta(0,j)\|_2 \\
     \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]}\int_{t}^{t+\tau} \int_{0}^{s} \|\nabla_{\vtheta} \Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j)) \|_2 \, du \, ds  \leq \tau T \cdot \sup_{t \in [0,T]} \max_{j \in [n]}  \|\nabla_{\vtheta} \Psi_{\lambda}(\vtheta(t,j); \rho^{\vtheta}(t,j)) \|_2 
\end{align*}

From Lemma \ref{lemma:noisy,bd,MFODE}, we know that:
\begin{align}
    \sup_{t \in [0,T]} \max_{j \in [n]}  \|\vtheta(s,j) - \vtheta(0,j)\|_2 \leq 2 \sup_{t \in [0,T]} \max_{j \in [n]}  \|\vtheta(s,j)\|_2 \leq K(\gamma,\lambda,\beta,T) (\sqrt{D+1+\log n + \delta^2}) \label{equ:Lip,noisy,7}
\end{align}
and 
\begin{align}
    \sup_{t \in [0,T]} \max_{j \in [n]}  \|\nabla_{\vtheta} \Psi_{\lambda}(\vtheta(t,j); \rho^{\vtheta}(t,j)) \|_2 & \leq  \sup_{t \in [0,T]} \max_{j \in [n]} K(1+|w_2(t,j)|) + \lambda \|\vtheta(t,j)\|_2 \notag \\
    & \leq K(\gamma,\lambda,\beta,T) (\sqrt{D+1+\log n + \delta^2}) \label{equ:Lip,noisy,8}
\end{align}

Thus now we remain to bound:
\begin{align*}
    \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2
\end{align*}

% We remark that the proof follows from Lemma \ref{lemma:bd,standard brownian}, since the standard $D+1$-dimensional Brownian have independent increments, which means that for any $k$, $\int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \,d \mB_j(s) $ is a Gaussian random variable, with covariance matrix: $2 \gamma \beta^{-1} h I$. Also, we have that for any $k \neq k'$, $\int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \,d \mB_j(s) $ and $\int_{k' \tau}^{k' \tau+h} \sqrt{2 \gamma \beta^{-1}} \,d \mB_j(s) $ are independent.

% Thus following from Lemma \ref{lemma:bd,standard brownian} we have:
% \begin{align*}
%     \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \, d \mB_j(s) \right\|_2 \leq 2 \sqrt{\lambda \beta^{-1} \tau}  \sqrt{D+ \log \left( n \lfloor \frac{T}{\tau} \rfloor \right) + \delta^2} 
% \end{align*}
% with probability at least $1 - \exp(-\delta^2)$

% Following the proof of Lemma \ref{lemma:bd,standard brownian}, we know that for any $u>0$,
% \begin{align*}
%   \Pr \left[\max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}}  \mB_j(s)\, ds \right\|_2 \geq u \tau \right] \leq  \Pr \left[ \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \, d \mB_j(s) \right\|_2 \geq u \right] 
% \end{align*}


% We aim to bound the following quantity:
% \begin{align*}
%      \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2 
% \end{align*}
% where $\{\mB_j(s)\}_{j \in [n]}$ are $n$ i.i.d standard $D$ -dimensional  Brownian motion. 

% We want to show that this quantity is upper bounded by $K(\gamma,T) \tau$.

By following the previous methods, we first consider to upper bound:
\begin{align*}
    \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2
\end{align*}
We have for any $u>0$
\begin{align*}
    &\left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2 \geq u \tau \\
    \Rightarrow &  \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \left\|\mB_j(s) \right\|_2 \, ds  \geq u \tau \\
    \Rightarrow & \sup_{h \in [0,\tau]} \sqrt{2 \gamma \beta^{-1}} \left\|\mB_j(k \tau+h) \right\|_2 \geq u
\end{align*}
Since the above holds for all $k \in \{1,...,\lfloor T / \tau \rfloor\},j \in [n]$, we have :
\begin{align*}
    &\max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2 \geq u \tau \\
    \Rightarrow &\max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]} \sup_{h \in [0,\tau]} \sqrt{2 \gamma \beta^{-1}} \left\|\mB_j(k \tau+h) \right\|_2 \geq u
\end{align*}
which implies that: 
\begin{align}
    &\Pr\left[ \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]} \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2 \geq u \tau \right] \\
    \leq & \Pr \left[\max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in [0,\tau]} \sqrt{2 \gamma \beta^{-1}} \left\|\mB_j(k \tau +h) \right\|_2 \geq u \right] \label{equ:Lip,noisy,10}
\end{align}

So now we aim to bound $\Pr \left[\max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in [0,\tau]} \sqrt{2 \gamma \beta^{-1}} \left\|\mB_j(k \tau +h) \right\|_2 \geq u \right]$.

In order to simplify the notation, we define $\overline{ \mB_j}(t) = \sqrt{2 \gamma \beta^{-1}} \mB_j(t)$

By the properties of standard Brownian motion, we have that $\overline{ \mB_j}(t)$ is a $D+1$-dimensional Gaussian random variable, with covariance matrix $2 \gamma \beta^{-1} t I_{D+1}$. Also since $\exp( \xi \| \overline{ \mB_j}(t)\|_2 )$ is a sub-martingale for any $\xi > 0$, following the same procedure in \cite[Proof of Lemma 13]{mei2019mean} we have:
\begin{align*}
    \Pr \left[ \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2 \geq u \right] &\leq (1- 2\xi \gamma \beta^{-1} (k+1)\tau )^{- (D+1)/2} \exp(- \xi u^2/2) \\
    & \leq (1- 2\xi \gamma \beta^{-1} T )^{- (D+1)/2} \exp(- \xi u^2/2)
\end{align*}
where the last step is due to the fact that $(k+1)\tau \leq T$ for $k \in \left\{ 0,1, ..., \lfloor \frac{T}{\tau} \rfloor \right\}$

By taking a union bound with respect to $k \in \left\{ 0,1, ..., \lfloor \frac{T}{\tau} \rfloor \right\}$ and $j \in [n]$, and take:
\begin{align*}
    &\xi = \frac{1}{4 \gamma^{-1} \beta T} \\
    &u = 2 \sqrt{\gamma^{-1} \beta T}  \sqrt{D+1+\log n\lfloor \frac{T}{\tau} \rfloor}
\end{align*}
we have:
\begin{align*}
    \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in [0,\tau]} \sqrt{2 \gamma \beta^{-1}} \left\|\mB_j(k \tau +h) \right\|_2 \leq 2 \sqrt{\gamma^{-1} \beta T}  \sqrt{D+1+\log n\lfloor \frac{T}{\tau} \rfloor} 
\end{align*}
with probability at least $1-\exp(-\delta^2)$

Thus by (\ref{equ:Lip,noisy,10}) we know that:
\begin{align}
     \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]} \sup_{h \in[0,\tau]} \left\| \int_{k \tau}^{k \tau+h} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2 \leq  2 \sqrt{\gamma^{-1} \beta T}  \sqrt{D+1+\log n\lfloor \frac{T}{\tau} \rfloor} \tau \label{equ:Lip,noisy,9}
\end{align}
with probability at least $1-\exp(-\delta^2)$

Now invoke (\ref{equ:Lip,noisy,7}), (\ref{equ:Lip,noisy,8}), (\ref{equ:Lip,noisy,9}) back to (\ref{equ:Lip,noisy,full}),and apply \ref{lemma:Pachatte}, we have that:
\begin{align*}
    \max_{k \in \left[\frac{T}{\tau}\right]}   \max_{j \in [n]}  \sup_{h \in[0,\tau]} \| \vtheta(t+\tau,j) - \vtheta(t,j) \|_2 \leq K(\gamma,\lambda,\beta,T) (\sqrt{D+1+\log n + \delta^2}) \tau
\end{align*}
with probability at least $1- \exp(-\delta^2)$


Now we are ready to proof Proposition \ref{prop:noisy,MFODE-PD}

\begin{proof}[Proof of Proposition \ref{prop:noisy,MFODE-PD}]
We only state the difference between the proof of noiseless case.

From the definition of the mean-field dynamics, we clearly have:
\begin{align*}
    \| \vtheta(t,j) - \vthetapd(t,j)\|_2 \leq \gamma \int_0^t \|\vtheta(s,j) - \vthetapd(s,j)\|_2 + \int_0^t \int_0^s \|\nabla_{\vtheta} \Psi_{\lambda} (\vtheta(u); \rho^{\vtheta}(u) ) - \nabla_{\vtheta} \Psi_{\lambda} (\vthetapd(u,j); \rhopd^{\vtheta}(u) )   \|_2 \, du \, ds
\end{align*}
Note that the Brownian noise terms are canceled since we coupled the Brownian motion to be the same. 

Following the same procedure as in Proof of Proposition \ref{prop:MFODE-PD,2L}, we have:
\begin{align}
    &\|\nabla_{\vtheta} \Psi_{\lambda} (\vtheta(u); \rho^{\vtheta}(u) ) - \nabla_{\vtheta} \Psi_{\lambda} (\vthetapd(u,j); \rhopd^{\vtheta}(u) )   \|_2 \notag \\
    \leq &  \|\nabla_{\vtheta} \Psi (\vtheta(u); \rho^{\vtheta}(u) ) - \nabla_{\vtheta} \Psi (\vthetapd(u,j); \rhopd^{\vtheta}(u) )   \|_2 \notag \\
    & + \lambda \|\vtheta(u) - \vthetapd(u,j) \|_2 \notag \\
    \leq & \|\nabla_{\vtheta} \Psi (\vtheta(u); \rho^{\vtheta}(u) ) - \nabla_{\vtheta} \Psi (\vtheta(u,j); \widehat{\rho}^{\vtheta}(u) )   \|_2  \label{equ:noisy,MFODE-PD,12}\\
    & + \|\nabla_{\vtheta} \Psi (\vtheta(u);  \widehat{\rho}^{\vtheta}(u) ) - \nabla_{\vtheta} \Psi (\vthetapd(u,j); \rhopd^{\vtheta}(u) )   \|_2 \label{equ:noisy,MFODE-PD,13}\\
    & + \lambda \|\vtheta(u) - \vthetapd(u,j) \|_2 \label{equ:noisy,MFODE-PD,14}
\end{align}
where as defined in the noiseless case, $\widehat{\rho}^{\vtheta}(t) = \frac{1}{n} \sum_{j=1}^n \delta_{\vtheta(t,j)} $ is the empirical distribution of the $n$-i.i.d mean-field dynamics.


For term \ref{equ:noisy,MFODE-PD,12}, we similarly use concentration inequality to bound it. Note that similar to the noiseless case, we have :
\begin{align*}
    &\sup_{t \in [0,T]} \max_{j \in [n]} \|\nabla_{\vtheta} \Psi (\vtheta(u); \rho^{\vtheta}(u) ) - \nabla_{\vtheta} \Psi (\vtheta(u,j); \widehat{\rho}^{\vtheta}(u) )   \|_2\\
    \leq & K (1 + |w_2(u,j)|) \cdot |\E_{\vx} f(\vx,\widehat{\rho}^{\vtheta}(u) ) - \E_{\vx}f(\vx,\rho^{\vtheta}(u) )| \\
    \leq &  K \left(1 +\sup_{t \in [0,T]} \max_{j \in [n]} |w_2(u,j)| \right) \cdot \sup_{t \in [0,T]}|\E_{\vx} f(\vx,\widehat{\rho}^{\vtheta}(u) ) - \E_{\vx}f(\vx,\rho^{\vtheta}(u) )| 
\end{align*}
where by definition:
\begin{align*}
    f(\vx,\widehat{\rho}^{\vtheta}(u) ) - f(\vx,\rho^{\vtheta}(u)= \frac{1}{n} \sum_{j=1}^n w_2(u,j) \sigma(\vw_1(u,j)^T \vx) - \E_{\rho^{\vtheta}(u)} w_2 \sigma(\vw_1^T \vx)
\end{align*}

Since from Lemma \ref{lemma:noisy,bd,MFODE} we know that:
\begin{align}
    \sup_{t \in [0,T]} \max_{j \in [n]} |w_2(t,j)| \leq (K T^2 + 2 T \sqrt{\lambda \beta^{-1} T}) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} T \right)  (\sqrt{1+\log n + \delta^2}) \label{equ:noisy,bdcondition,MFODE}
\end{align}
with probability at least $1- \exp(-\delta^2)$



For simplicity of the notations, we define the following events:
\begin{align*}
    & \mathcal{E}_1 = \left\{ \sup_{t \in [0,T]} \max_{j \in [n]} |w_2(t,j)| \geq (K T^2 + 2 T \sqrt{\lambda \beta^{-1} T}) \exp\left( \frac{\gamma^2 + \lambda^2}{\gamma} T \right)  (\sqrt{1+\log n + \delta^2})  \right\}
\end{align*}

We also define:
\begin{align*}
    Q(u) = \left|\frac{1}{n} \sum_{j=1}^n  w_2(u,j) \sigma(\vw_1(u,j)^T \vx) - \E_{\rho^{\vtheta}(u)} w_2 \sigma(\vw_1^T \vx) \right| 
\end{align*}

and we aim to bound $\sup_{u \in [0,T]} Q(u)$. 


From now on, all the events we state are condition on  $\overline{\mathcal{E}_1}$.

We have:
\begin{align*}
   |w_2(u,j) \sigma(\vw_1(u,j)^T \vx) - \E_{\rho^{\vtheta}(u)} w_2 \sigma(\vw_1^T \vx)| \leq K(\gamma,\lambda,\beta,T) (\sqrt{1+\log n + \delta^2})
\end{align*}


And by Lemma \ref{lemma:Corollary of McDiarmid inequality}, we have:
\begin{align*}
    Q(t) \leq K(\gamma,\lambda,\beta,T) (\sqrt{1+\log n + \delta^2}) \left( \frac{1}{\sqrt{n}} + \delta' \right)
\end{align*}


For simplicity of the notation, we denote the event:
\begin{align*}
    \mathcal{E}_2 =  \left\{ Q(t) \geq K(\gamma,\lambda,\beta,T) (\sqrt{1+\log n + \delta^2}) \left( \frac{1}{\sqrt{n}} + \delta' \right) \right\}
\end{align*}with probability $1 - \exp(n \delta')$.

Now we aim to  take  a union bound w.r.t time $t \in \{0,1,..., \lfloor T/\eta \rfloor \}$, by Lemma \ref{lemma:Lip,noisy,2L}  we have:
\begin{align}
    & \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]} |Q(k \tau + h) - Q(k \tau) | \notag \\
    \leq &   \frac{1}{n} \sum_{j=1}^{n} \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}| w_2(k \tau + h,j) \sigma(\vw_1(k \tau + h,j)^T \vx) -  w_2(k \tau ,j) \sigma(\vw_1(k \tau ,j)^T \vx)| \label{equ:noisy,Lip,w} \\
    & + \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]} |\E_{\rho^{\vtheta}(k \tau + h)} w_2 \sigma(\vw_1^T \vx)  - \E_{\rho^{\vtheta}(k \tau)} w_2 \sigma(\vw_1^T \vx) | \label{equ:noisy,Lip,rho}
\end{align}

For term (\ref{equ:noisy,Lip,w}), we have:
\begin{align*}
     & \frac{1}{n} \sum_{j=1}^{n} \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}| w_2(k \tau + h,j) \sigma(\vw_1(k \tau + h,j)^T \vx) -  w_2(k \tau ,j) \sigma(\vw_1(k \tau ,j)^T \vx)| \\
     \leq & \max_{j \in [n]} \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}| w_2(k \tau + h,j) \sigma(\vw_1(k \tau + h,j)^T \vx) -  w_2(k \tau ,j) \sigma(\vw_1(k \tau ,j)^T \vx)| \\
     \leq & K \left(1+  \max_{j \in [n]} \sup_{t \in [0,T]} | w_2(t,j)|  \right) \cdot  \max_{j \in [n]} \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}  \| \vtheta(k \tau + h,j) - \vtheta(k \tau, j)\|_2
\end{align*}

For simplicity we define 
\begin{align*}
    Q_1 = \frac{1}{n} \sum_{j=1}^n \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}  \left|w_2(k \tau+h,j) \sigma(\vw_1(k \tau+h,j)^T \vx)   - w_2(k \tau,j) \sigma(\vw_1(k \tau,j)^T \vx)  \right|
\end{align*}


By Lemma \ref{lemma:noisy,bd,MFODE} and Lemma \ref{lemma:Lip,noisy,2L}, we have:
\begin{align*}
     & \max_{j \in [n]} \sup_{t \in [0,T]} | w_2(t,j)|  \leq K(\gamma,\lambda, \beta, T) \sqrt{1+\log n+ \delta^2} \\
     & \max_{j \in [n]} \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}  \| \vtheta(k \tau + h,j) - \vtheta(k \tau, j)\|_2 \leq K(\gamma,\lambda, \beta, T) \sqrt{D+1+\log n+ \delta^2} \tau
\end{align*}
with probability at least $1- \exp(- \delta^2)$, which implies that:
\begin{align}
     Q_1 \leq  K(\gamma,\lambda, \beta, T) \left( D+1+\log n+ \delta^2 \right) \cdot \tau \label{equ:Lip,noisy,Q_1}
\end{align}
with probability at least $1- \exp(- \delta^2)$

 For simplicity, we define event:
 \begin{align*}
     \mathcal{E}_3 = \left\{ Q_1
    \geq  K(\gamma,\lambda, \beta, T) \left( D+1+\log n+ \delta^2 \right) \cdot \tau \right\}
 \end{align*}

For term (\ref{equ:noisy,Lip,rho}), we have:
\begin{align*}
    & \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]} |\E_{\rho^{\vtheta}(k \tau + h)} w_2 \sigma(\vw_1^T \vx)  - \E_{\rho^{\vtheta}(k \tau)} w_2 \sigma(\vw_1^T \vx) | \\
    \leq &  \E \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]} \left|w_2(k \tau+h,j) \sigma(\vw_1(k \tau+h,j)^T \vx)   - w_2(k \tau,j) \sigma(\vw_1(k \tau,j)^T \vx)  \right| , \forall j \in [n]  \\
    \leq & \E \left[ \frac{1}{n} \sum_{j=1}^n \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]}  \left|w_2(k \tau+h,j) \sigma(\vw_1(k \tau+h,j)^T \vx)   - w_2(k \tau,j) \sigma(\vw_1(k \tau,j)^T \vx)  \right|  \right] \\
    = & \E[Q_1] =  \int_{0}^{+\infty}  \Pr [Q_1 \geq u] \, du 
\end{align*}

Note that $\left( D+1+\log n+ \delta^2 \right) \geq \frac{1}{2} \left(   \sqrt{D+1+\log n}+ \delta \right)^2$, so we have:
\begin{align*}
    \Pr \left[Q_1 \geq \frac{1}{2} K(\gamma,\lambda,\beta, T) \left(   \sqrt{D+1+\log n}+ \delta \right)^2 \cdot \tau \right] \leq \exp(-\delta^2)
\end{align*}

Note that:
\begin{align*}
    \E[Q_1] =  K(\gamma,\lambda,\beta, T)\cdot \tau \E\left[\frac{Q_1}{ K(\gamma,\lambda,\beta, T)\cdot \tau} \right]
\end{align*}
and we denote $\overline{Q_1} =\frac{Q_1}{ K(\gamma,\lambda,\beta, T)\cdot \tau} $

By doing a change of variable, let $\xi = \sqrt{D+1+\log n}+ \delta$, we have:
\begin{align*}
    \E[\overline{Q_1}] \leq & \int_{0}^{+ \infty} \Pr[\overline{Q_1} \geq u] \, du \\
    \leq & \int_{- \sqrt{D+1+\log n} }^{+ \infty} \xi \exp(- (\xi-\sqrt{D+1+\log n})^2) \, d\xi \\
    \leq & \frac{1}{2} (\sqrt{2 \pi} \sqrt{D+1+\log n}+1)
\end{align*}
which implies that:
\begin{align}
    \E[Q_1] \leq  K(\gamma,\lambda,\beta, T)  \frac{1}{2} (\sqrt{2 \pi} \sqrt{D+1+\log n}+1)  \tau \label{equ:Lip,noisy,E[Q_1]}
\end{align}

Thus combining (\ref{equ:Lip,noisy,Q_1}) and (\ref{equ:Lip,noisy,E[Q_1]}), and absorbing lower order terms w.r.t $n,D$ we have that:
\begin{align*}
    \max_{k \in [ \lfloor T/ \varepsilon \rfloor] } \sup_{h \in [0,\tau]} |Q(k \tau + h) - Q(k \tau) | \leq K(\gamma,\lambda, \beta, T) \left( D+1+\log n+ \delta^2 \right) \cdot \tau 
\end{align*}
with probability at least $1 - \exp(-\delta^2)$

Thus by taking union bound w.r.t $k \in \{0,1,..., \lfloor \frac{T}{\eta} \rfloor \}$ we have that:
\begin{align*}
     \sup_{t \in [0,T]} Q(t) \leq   K(\gamma,\lambda,\beta,T) (\sqrt{1+\log n + \delta^2}) \left( \frac{1}{\sqrt{n}} + \delta' \right) +  K(\gamma,\lambda, \beta, T) \left( D+1+\log n+ \delta^2 \right) \cdot \eta  
\end{align*}
with probability at least $1 - \lfloor \frac{T}{\eta} \rfloor  \exp(- n \delta'^2) $ 

Take $\eta = \frac{1}{\sqrt{n}}$ and $\delta' = \frac{\log \sqrt{n}T + \delta^2}{ \sqrt{n}}$, and absorbing lower order terms w.r.t $n,D$, we have:
\begin{align*}
     \sup_{t \in [0,T]} Q(t) \leq   K(\gamma,\lambda,\beta,T) \left[ (\sqrt{1+\log n + \delta^2}) \frac{\log \sqrt{n}T + \delta^2}{ \sqrt{n}} +   \left( D+1+\log n+ \delta^2 \right) \frac{1}{\sqrt{n}} \right]
\end{align*}
with probability at least $1 -\exp(-\delta^2)$

For simplicity, we define $ \err(\delta) =  K(\gamma,\lambda,\beta,T) \left[ (\sqrt{1+\log n + \delta^2}) \frac{\log \sqrt{n}T + \delta^2}{ \sqrt{n}} +   \left( D+1+\log n+ \delta^2 \right) \frac{1}{\sqrt{n}} \right]$ and denote that event:
\begin{align*}
    \mathcal{E}_4 = \{ \sup_{t \in [0,T]} Q(t) \geq  \err(\delta)\}
\end{align*}

From the above analysis, we know that:
\begin{align*}
    \Pr [\mathcal{E}_1], \Pr [\mathcal{E}_2 |\overline{\mathcal{E}_1 } ] , \Pr [\mathcal{E}_3 |\overline{\mathcal{E}_1 } ], \Pr [\mathcal{E}_4 |\overline{\mathcal{E}_1 },\overline{\mathcal{E}_2 },\overline{\mathcal{E}_3 } ] \leq \exp(- \delta^2)
\end{align*}
which implies that:
\begin{align*}
    \Pr [\mathcal{E}_4] \leq 6 \exp(- \delta^2)
\end{align*}
\end{proof}
%----------------------------------------------------------------------------------
% \textcolor{blue}{An alternative way to bound it is as follows:}


% Now we aim to bound $\Pr \left[ \max_{k \in \left[\frac{T}{\tau}\right]} \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2 \geq u \right]$

%  %We define the filtration generated by $\left\{\left\|\overline{\mB}_j(i \tau + h) \right\|_2: i \leq k \right\}$ as $\mathcal{F}_k(h)$, we define $\mathcal{F}_k = \cup_{h \in [0,\tau]} \mathcal{F}_k(h)$ 

% We claim that $Y_k = \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2$  is a sub-martingale. 

% First note that $\left\|\overline{\mB}_j(t) \right\|_2$ is a sub-martingale  since $\L_2$ norm is convex and $\overline{\mB}_j(t)$ is a martingale.

% We claim that  $Y_k = \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2$ is still a sub-martingale.

% To state the result, we first define $\mathcal{F}_k$ be the filtration generated by $Y_0,...,Y_k$. Then , it is easy to see that we have : $\E \left[Y_{k+1} \big| \mathcal{F}_k \right] \geq & Y_k$ since $\left\|\overline{\mB}_j(t) \right\|_2$ is a sub-martingale for any $t$.

% Thus by applying the Doob's martingale inequality, we have:
% \begin{align*}
%     \Pr \left[ \max_{k \in \left[\frac{T}{\tau}\right]} \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2 \geq u \right] \leq \frac{\E \left[ \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(T- \tau +h) \right\|_2  \right]}{u}
% \end{align*}

% Since we know that:
% \begin{align*}
%     \Pr \left[ \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2 \geq u \right] &\leq (1- 2\xi \gamma \beta^{-1} (k+1)\tau )^{- (D+1)/2} \exp(- \xi u^2/2) \\
%     & \leq (1- 2\xi \gamma \beta^{-1} T )^{- (D+1)/2} \exp(- \xi u^2/2)
% \end{align*}
% we have:
% \begin{align*}
%     &\E \left[ \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(T- \tau +h) \right\|_2  \right] \\
%     \leq & \int_{-\infty}^{\infty}  \Pr \left[ \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2 \geq u \right]  \,du \\
%     \leq  & (1- 2\xi \gamma \beta^{-1} T )^{- (D+1)/2} \int_{-\infty}^{\infty} \exp(- \xi u^2/2) \, du\\
%     =& (1- 2\xi \gamma \beta^{-1} T )^{- (D+1)/2} \sqrt{\frac{\xi}{2 \pi}}
% \end{align*}
% and thus implies that:
% \begin{align*}
%     \Pr \left[ \max_{k \in \left[\frac{T}{\tau}\right]} \sup_{h \in [0,\tau]} \left\|\overline{\mB}_j(k \tau +h) \right\|_2 \geq u \right] \leq (1- 2\xi \gamma \beta^{-1} T )^{- (D+1)/2} \cdot \sqrt{\frac{\xi}{2 \pi}} \cdot \frac{1}{u}
% \end{align*}

% By taking a union
%----------------------------------------------------------------------------
% 
% Now note that by definition $\overline{\mB}_j$ are i.i.d standard Brownian, so we can take union bounds w.r.t $n$



%  Similarly, we first aim to give an upper bound on $\max_{j \in [n]} \| \vtheta(t,j) - \vtheta(0,j) \|_2 $, we have:
% \begin{align*}
%     \| \vtheta(t,j) - \vtheta(0,j) \|_2 \leq  \gamma \int_{0}^{t} \|\vtheta(s,j) - \vtheta(0,j)\|_2 \, ds + \int_{0}^{t} \int_{0}^{s} \nabla_{\vtheta} \|\Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j))\|_2 \,du \,ds \\
%     \hspace{17em} + \sqrt{2 \gamma \beta^{-1}} \left\| \int_{0}^{t} \mB_j(s) \, ds \right\|_2,
% \end{align*}
% which implies that:
% \begin{align}
%     \max_{j \in [n]} \| \vtheta(t,j) - \vtheta(0,j) \|_2 \leq  \gamma \int_{0}^{t} \max_{j \in [n]} \|\vtheta(s,j) - \vtheta(0,j)\|_2 \, ds + \int_{0}^{t} \int_{0}^{s} \max_{j \in [n]}  \|\nabla_{\vtheta} \Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j))\|_2 \,du \,ds  \notag \\
%     \hspace{13 em}+  \max_{j \in [n]} \left\| \int_{0}^{t} \sqrt{2 \gamma \beta^{-1}} \mB_j(s) \, ds \right\|_2, \label{equ:Lip,noisy,1}
% \end{align}

% By Lemma \ref{lemma:priori,2L,noisy}, we have that:
% \begin{align*}
%     \nabla_{\vtheta} \|\Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j))\|_2 \leq K(1+\|w_2(t,j)\|_2)+ \lambda \|\vtheta(t,j)\|_2
% \end{align*}
% which implies that:
% \begin{align*}
%     \max_{j \in [n]} \|\Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j))\|_2 \leq K(1+\max_{j \in [n]} \|w_2(t,j)\|_2)+ \lambda \max_{j \in [n]} \|\vtheta(t,j)\|_2
% \end{align*}

% By using the same methods as in \cite[Lemma 13]{mei2019mean}, we have:
% \begin{align*}
%     \max_{j \in [n]} \|w_2(t,j)\|_2 \leq \max_{j \in [n]} \|\vtheta(t,j)\|_2 \leq K(\gamma, \lambda, \beta, T) \big( \sqrt{D+1+\log n} + \delta \big)
% \end{align*}
% with probability at least $1-\exp(-\delta^2)$

% Thus we have :
% \begin{align*}
%      \max_{j \in [n]} \|\nabla_{\vtheta} \Psi_{\lambda}(\vtheta(u,j); \rho^{\vtheta}(u,j))\|_2 \leq K(\gamma, \lambda, \beta, T) \big( \sqrt{D+1+\log n} + \delta \big)
% \end{align*}
% with probability at least $1-\exp(-\delta^2)$

% For the $ \max_{j \in [n]} \left\| \int_{0}^{t} \sqrt{2 \gamma \beta^{-1}}\mB_j(s) \, ds \right\|_2$ term, from Lemma \ref{lemma:bd,standard brownian}, we have:
% \begin{align*}
%     \max_{j \in [n]} \left\| \int_{0}^{t} \sqrt{2 \gamma \beta^{-1}}\mB_j(s) \, ds \right\|_2 \leq 2 T \sqrt{ \gamma \beta^{-1} T }\sqrt{D+1+\log n + \delta^2}
% \end{align*}
% with probability at least $1-\exp(-\delta^2)$.

% Thus, invoking the above into (\ref{equ:Lip,noisy,1}), we have:
% \begin{align*}
%     \max_{j \in [n]} \| \vtheta(t,j) - \vtheta(0,j) \|_2 \leq  \gamma \int_{0}^{t} \max_{j \in [n]} \|\vtheta(s,j) - \vtheta(0,j)\|_2 \, ds +K(\gamma, \lambda, \beta, T)  \sqrt{D+1+\log n + \delta^2} 
% \end{align*}
% and by Gronwall's lemma we have:
% \begin{align*}
%     \max_{j \in [n]} \| \vtheta(t,j) - \vtheta(0,j) \|_2 \leq K(\gamma, \lambda, \beta, T) \exp(\gamma T)  \sqrt{D+1+\log n + \delta^2} 
% \end{align*}

% Now we a ready to prove the main result. By the definition of the mean-field dynamics, we have :

\end{proof}



==> 2_layers/noisy_PD-HB.tex <==
We recall that the noisy heavy ball dynamics is defined as in (\ref{equ:noisy,HB})

And the noisy particle dynamics is defined as in (\ref{equ:noisy,PD}).

\begin{proposition}




\end{proposition}

==> 2_layers/priori_estimation_2L_noisy.tex <==
\textcolor{red}{Similarly, may be clearer as two separate Lemmas}
\begin{lemma}
\label{lemma:priori,2L,noisy}
Consider $T>0$ and $t \leq T$. Under assumption \ref{Assum:2L} and with $f(\vx;\rho), \Psi_{\lambda}(\vtheta;\rho), \nabla_{\vtheta} \Psi_{\lambda}(\vtheta;\rho)$ as defined in (\ref{equ:defMF,2L}), we have that: 

\begin{enumerate}
    \item (Boundedness) We have that, for any $\vtheta, \rho$:
    \begin{equation}
        \begin{split}
            &f(\vx;\rho) \leq K \E_{\rho}|w_2|, \\
            &|\Psi_{\lambda}(\vtheta;\rho)| \leq K |w_2| + \frac{\lambda}{2} (\|\vw_1\|_2^2+ |w_2|^2), \\
            &\|\nabla_{\vw_1} \Psi_{\lambda}(\vtheta;\rho)\|_2 \leq K |w_2| + \lambda \|\vw_1\|_2\\
            &\|\nabla_{w_2} \Psi_{\lambda}(\vtheta;\rho)\|_2 \leq K  + \lambda |w_2|
        \end{split}
    \end{equation}
    
    \item (Boundedness of the mean-field ODE) 
    \begin{equation}
        |w_2(t)| \leq K(\gamma, \lambda, \beta,T) (1+ \delta)
    \end{equation}
    and 
    \begin{equation}
        \|\vw_1(t)\|_2 \leq K(\gamma, \lambda, \beta,T) (\sqrt{D}+ \delta)
    \end{equation}
    with probability at least $ 1 - \exp(-\delta^2)$, where $K(\gamma, \lambda, \beta,T)$ are universal constant that only depends on $\gamma, \lambda, \beta,T$.
    Also:
    \begin{equation}
        \|\vtheta(t)\|_2 \leq K(\gamma, \lambda, \beta,T) ( \sqrt{D+ 1}+ \delta)
    \end{equation}
    % \begin{equation}
    %     \|\vw_1(t)\|_2 \leq 
    % \end{equation}
    
    \item (Lipschitz continuity): 
    \begin{align}
        |\Psi_{\lambda}(\vtheta;\rho) - \Psi_{\lambda}(\vtheta';\rho')| \leq K(1+ |w_2|) \left(|w_2-w_2'| + \|\vw_1 - \vw'_1\|_2 + \wass_2(\rho,\rho')\right) + \frac{\lambda}{2} \big(\|\vtheta\|^2_2 -  \|\vtheta'\|^2_2 \big)\\
        \|\nabla_{\theta}\Psi_{\lambda}(\vtheta;\rho) - \nabla_{\theta}\Psi_{\lambda}(\vtheta';\rho')\|_2 \leq K(1+ |w_2|) \left(|w_2-w_2'| + \|\vw_1 - \vw'_1\|_2 + \wass_2(\rho,\rho')\right) + \frac{\lambda}{2} \big\|\vtheta-\vtheta'\big\|_2
    \end{align}
\end{enumerate}

\end{lemma}

\begin{proof}
\begin{enumerate}
    \item For the boundedness, the proof is the same as the proof for Lemma \ref{lemma:priori,2L}.
    
    \item For the boundedness of the mean-field ODE, we note that by the definition of the mean-field ODE:
    \begin{align*}
        w_2(t) = w_2(0) - \gamma \int_{0}^{t} (w_2(s) - w_2(0)) \, ds - \int_{0}^{t} \int_{0}^{s} \nabla_{w_2} \Psi_{\lambda}(\vtheta(u);\rho^{\vtheta}(u)) \, du \, ds - \sqrt{2 \gamma \beta^{-1}} \int_{0}^{t} B(s) \, ds
    \end{align*}
    where  
    \begin{align*}
        &\nabla_{w_2} \Psi_{\lambda}(\vtheta(u);\rho^{\vtheta}(u)) =\E_{\vz}\left[ \partial_2 R(y,f(\vx;\rho(u))) \sigma(\vw_1(u)^T \vx)\right] + \frac{\lambda}{2} w_2\\
        % &\nabla_{\vw_1} \Psi_{\lambda}(\vtheta(u);\rho^{\vtheta}(u)) = \E_{\vz}\left[ \partial_2 R(y,f(\vx;\rho(u)))  w_2(u) \sigma'(\vw_1(u)^T \vx) \vx \right] + \frac{\lambda}{2} \vw_1
    \end{align*} and $B(s)$ is a one-dimensional standard Brownian motion.
    
    Hence we have:
    \begin{align*}
        |w_2(t)|  \leq & |w_2(0)| + \gamma \int_{0}^{t} |w_2(s)| + |w_2(0)| \, ds \\
        & +\int_{0}^{t} \int_{0}^{s} |\E_{\vz}\left[ \partial_2 R(y,f(\vx;\rho(u))) \sigma(\vw_1(u)^T \vx)\right]| + \frac{\lambda}{2} |w_2| \, du \, ds + \left| \int_{0}^{t} \sqrt{2 \gamma \beta^{-1}} B(s) \, ds \right|\\
        \leq & (K + KT + K T^2) + \gamma \int_{0}^{t} |w_2(s)|  \, ds  + \frac{\lambda}{2} \int_{0}^{t} \int_{0}^{s}  |w_2(u)| \, du \, ds  + \left| \int_{0}^{t}\sqrt{2 \gamma \beta^{-1}} B(s) \, ds \right|
    \end{align*}
    for the $\left| \int_{0}^{t} B(s) \, ds \right|$ term, we have from Lemma \ref{lemma:bd,standard brownian} that:
    \begin{align*}
        \left| \int_{0}^{t} B(s) \, ds \right| \leq \sup_{t \in [0,T]} \left| \int_{0}^{t} B(s) \, ds \right| \leq   KT \sqrt{\lambda \beta^{-1} T} (1+\delta)
    \end{align*}
    with probability at least $1 - \exp(-\delta^2)$.
    
    Thus we have that:with probability at least $1 - \exp(-\delta^2)$
   \begin{align*}
        |w_2(t)|  \leq  (K T^2 + KT \sqrt{\lambda \beta^{-1} T} (1+\delta)) + \gamma \int_{0}^{t} |w_2(s)|  \, ds  + \frac{\lambda}{2} \int_{0}^{t} \int_{0}^{s}  |w_2(u)| \, du \, ds 
    \end{align*}
    which by Lemma \ref{lemma:Pachatte} implies that:
    \begin{align*}
        |w_2(t)| \leq (K T^2 + KT \sqrt{\lambda \beta^{-1} T} ) \left(1 + \exp\left( \frac{\gamma^2 + \lambda}{\gamma}T\right) \right) (1+\delta) : = K(\gamma, \lambda, \beta,T) (1+ \delta)
    \end{align*}
    where we define : $K(\gamma, \lambda, \beta,T) =(K T^2 + KT \sqrt{\lambda \beta^{-1} T} ) \left(1 + \exp\left( \frac{\gamma^2 + \lambda}{\gamma}T\right) \right) $, and it is a universal constant that only depends on $\gamma, \lambda, \beta,T $
    
    For the $\|\vw_1(t)\|_2$, note by the definition of the mean-field ODE we have:
    \begin{align*}
        \vw_1(t) = \vw_1(0) - \gamma \int_{0}^{t}( \vw_1(s) - \vw_1(0)) \, ds - \int_{0}^{t} \int_{0}^{s} \nabla_{\vw_1} \Psi_{\lambda}(\vtheta(u);\rho^{\vtheta}(u)) \, du \, ds + \sqrt{2 \gamma \beta^{-1}} \int_{0}^{t} \mB(s) \, ds
    \end{align*}
    where $\nabla_{\vw_1} \Psi_{\lambda}(\vtheta(u);\rho^{\vtheta}(u)) = \E_{\vz}\left[ \partial_2 R(y,f(\vx;\rho(u)))  w_2(u) \sigma'(\vw_1(u)^T \vx) \vx \right] + \frac{\lambda}{2} \vw_1$
    and $\mB(s)$ is a $D$-dimensional standard Brownian motion. 
    
    Hence we have:
    \begin{align*}
        \|\vw_1(t)\|_2 \leq & \|\vw_1(0)\|_2 + \gamma \int_{0}^{t} \|\vw_1(s)\|_2 + \|\vw_1(0)\|_2 \, ds \\
        &+ \int_{0}^{t} \int_{0}^{s} \left\|\nabla_{\vw_1} \Psi_{\lambda}(\vtheta(u);\rho^{\vtheta}(u)) \right\|_2 \, du \, ds + \sqrt{2 \gamma \beta^{-1}} \left\| \int_{0}^{t} \mB(s) \, ds \right\|_2
    \end{align*}
    
    Since by assumption \ref{Assum:2L}, we assume that $\vw_1(0)$ is a $D$-dimensional  $K$-sub-Gaussian. Following the same proof as in \cite[Lemma 13]{mei2019mean}, we have:
    \begin{align*}
        \|\vw_1(0)\|_2 \leq 2K \big( \sqrt{D} + \delta \big)
    \end{align*}
    with probability at least $1-\exp(-\delta^2)$, and similarly from Lemma \ref{lemma:bd,standard brownian} we have:
    \begin{align*}
        \sqrt{2 \gamma \beta^{-1}} \left\| \int_{0}^{t} \mB(s) \, ds \right\|_2 \leq 2T\sqrt{ \gamma \beta^{-1} T} \big( \sqrt{D+\delta^2}\big) 
    \end{align*}
    with probability at least $1 - \exp(-\delta^2)$. 
    
    Combining the above bounds for $\vw_1$, we have that:
    \begin{align*}
        \|\vw_1(t)\|_2 \leq & K(1+T)(\sqrt{D}+\delta) + \gamma \int_{0}^{t} \|\vw_1(s)\|_2  \, ds  \\
        & + \int_{0}^{t} \int_{0}^{s} K |w_2(u)| + \lambda |w_1(u)| \, du \, ds + 2T\sqrt{ \gamma \beta^{-1} T} \big( \sqrt{D+\delta^2}\big) 
    \end{align*}
    with probability at least $1-\exp(-\delta^2)$
    
    We know that $|w_2(u)| \leq K(\gamma,\lambda,\beta,T)(1+ \delta)$ with probability at least $1 - \exp(-\delta^2)$. Thus we have:
    \begin{align*}
        \|\vw_1(t)\|_2 \leq & (K(1+T)+2T\sqrt{ \gamma \beta^{-1} T})(\sqrt{D}+\delta) + K(\gamma,\lambda,\beta,T)(1+ \delta) \\
        &+ \gamma \int_{0}^{t} \|\vw_1(s)\|_2  \, ds + \lambda \int_{0}^{t} \int_{0}^{s}  |\vw_1(u)| \, du \, ds
    \end{align*}
    which by Lemma \ref{lemma:Pachatte} implies that:
    \begin{align*}
         \|\vw_1(t)\|_2 \leq K(\gamma,\lambda,\beta,T)(\sqrt{D}+\delta)
    \end{align*}
    with probability at least $1-\exp(-\delta^2)$
    
    \item For the Lipschitz continuity argument, it is also same as in the proof of Lemma \ref{lemma:priori,2L}, thus we omitted it here. 
\end{enumerate}
\end{proof}


